Quantum Monte Carlo study of ultracold gases (PhD thesis)

This Dissertation presents results of a thorough study of ultracold bosonic and fermionic gases in three-dimensional and quasi-one-dimensional systems. Although the analyses are carried out within various theoretical frameworks (Gross-Pitaevskii, Bethe ansatz, local density approximation, etc.) the main tool of the study is the Quantum Monte Carlo method in different modifications (variational Monte Carlo, diffusion Monte Carlo, fixed-node Monte Carlo methods). We benchmark our Monte Carlo calculations by recovering known analytical results (perturbative theories in dilute limits, exactly solvable models, etc.) and extend calculations to regimes, where the results are so far unknown. In particular we calculate the equation of state and correlation functions for gases in various geometries and with various interatomic interactions.

==> 1dhardrod.tex <==
%\begin{abstract}
%We consider a homogeneous 1D Bose gas with contact interactions and large attractive coupling constant. This system
%can be realized in tight waveguides by exploiting a confinement induced resonance of the effective 1D scattering
%amplitude. By using a variational {\it ansatz} for the many-body wavefunction, we show that for small densities
%the gas-like state is stable and the corresponding equation of state is well described by a gas of hard
%rods. By calculating the compressibility of the system, we provide an estimate of the critical density at which the
%gas-like state becomes unstable against cluster formation. Within the hard-rod model we calculate the one-body density
%matrix and the static structure factor of the gas. The results show that in this regime the system is more strongly
%correlated than a Tonks-Girardeau gas. The frequency of the lowest breathing mode for harmonically trapped systems is
%also discussed as a function of the interaction strength.
%\end{abstract}
\section{Introduction}

The study of quasi-1D Bose gases in the quantum-degenerate regime has become a very
active area of research. The role of correlations and of quantum fluctuations is
greatly enhanced by the reduced dimensionality and 1D quantum gases constitute well
suited systems to study beyond mean-field effects \cite{Petrov00}. Among these,
particularly intriguing is the fermionization of a 1D Bose gas in the strongly
repulsive Tonks-Girardeau (TG) regime, where the system behaves as if it consisted
of noninteracting spinless fermions \cite{Girardeau60}. The Bose-Fermi mapping of
the TG gas is a peculiar aspect of the universal low-energy properties which are
exhibited by bosonic and fermionic gapless 1D quantum systems and are described by
the Luttinger liquid model \cite{Voit95}. The concept of Luttinger liquid plays a
central role in condensed matter physics and the prospect of a clean testing for its
physical implications using ultracold gases confined in highly elongated traps is
fascinating \cite{Monien98,Recati03}.

Bosonic gases in 1D configurations have been realized experimentally. Complete
freezing of the transverse degrees of freedom and fully 1D kinematics has been
reached for systems prepared in a deep 2D optical lattice \cite{Moritz03,Tolra04}.
The strongly interacting regime has been achieved by adding a longitudinal periodic
potential and the transition from a 1D superfluid to a Mott insulator has been
observed \cite{Stoferle04}. A different technique to increase the strength of the
interactions, which is largely employed in both bosonic and fermionic 3D systems
\cite{Inouye98,O'Hara02} but has not yet been applied to 1D configurations, consists
in the use of a Feshbach resonance. With this method one can tune the effective 1D
coupling constant $g_{1D}$ to essentially any value, including $\pm\infty$, by
exploiting a confinement induced resonance \cite{Olshanii98,Bergeman03}. For large
and positive values of $g_{1D}$ the system is a TG gas of point-like impenetrable
bosons. On the contrary, if $g_{1D}$ is large and negative, we will show that a new
gas-like regime is entered (super-Tonks) where the hard-core repulsion between
particles becomes of finite range and correlations are stronger than in the TG
regime. In this Chapter we investigate using Variational Monte Carlo techniques
(\ref{secVMC}) the equation of state and the correlation functions of a homogeneous
1D Bose gas in the super-Tonks regime. We find that the particle-particle
correlations decay faster than in the TG gas and that the static structure factor
exhibits a pronounced peak. The momentum distribution and the structure factor of
the gas are directly accessible in experiments by using, respectively,
time-of-flight techniques and two-photon Bragg spectroscopy \cite{Stoferle04}. The
study of collective modes also provides a useful experimental technique to
investigate the role of interactions and beyond mean-field effects \cite{Moritz03}.
Within a local density approximation (LDA) for systems in harmonic traps we
calculate the frequency of the lowest compressional mode as a function of the
interaction strength in the crossover from the TG gas to the super-Tonks regime.

\section{The model and method}

We consider a 1D system of $N$ spinless bosons described by the following
contact-interaction Hamiltonian
%
\begin{equation}
H=-\frac{\hbar^2}{2m}\sum_{i=1}^{N}\frac{\partial^2}{\partial z_i^2}+g_{1D}\sum_{i<j}\delta(z_{ij}) \;,
\label{Hamiltonian}
\end{equation}
%
where $m$ is the mass of the particles, $z_{ij}=z_i-z_j$ denotes the interparticle
distance between particle $i$ and $j$ and $g_{1D}$ is the coupling constant which we
take large and negative. The study of the scattering problem of two particles in
tight waveguides yields the following result for the effective 1D coupling constant
$g_{1D}$ in terms of the 3D $s$-wave scattering length $a_{3D}$ \cite{Olshanii98} is
given by the formula (\ref{g1Dolshanii}), where $a_\perp=\sqrt{\hbar/m\omega_\perp}$
is the characteristic length of the transverse harmonic confinement producing the
waveguide. The confinement induced resonance is located at the critical value
$a_{3D}^c$ and corresponds to the abrupt change of $g_{1D}$ from large positive
values ($a_{3D}\lesssim a_{3D}^c$) to large negative values ($a_{3D}\gtrsim
a_{3D}^c$). The renormalization (\ref{g1Dolshanii}) of the effective 1D coupling
constant has been recently confirmed in a many-body calculation of Bose gases in
highly elongated harmonic traps using quantum Monte Carlo techniques
\cite{Astrakharchik04,Astrakharchik04c}.

For positive $g_{1D}$, the Hamiltonian (\ref{Hamiltonian}) corresponds to the
Lieb-Liniger (LL) model (\ref{LL}). The ground state and excited states of the LL
Hamiltonian have been studied in detail \cite{Lieb63,Lieb63b} and, in particular,
the TG regime corresponds to the limit $g_{1D}=+\infty$. The ground state of the
Hamiltonian (\ref{Hamiltonian}) with $g_{1D}<0$ has been investigated by McGuire
\cite{McGuire64} and one finds a soliton-like state with energy
$E/N=-mg_{1D}^2(N^2-1)/24\hbar^2$. The lowest-lying gas-like state of the
Hamiltonian (\ref{Hamiltonian}) with $g_{1D}<0$ corresponds to a highly-excited
state that is stable if the gas parameter $na_{1D}\ll 1$, where $n$ is the density
and $a_{1D}$ is the 1D effective scattering length defined in Eq.
(\ref{g1Dolshanii}). This state can be realized in tight waveguides by crossing
adiabatically the confinement induced resonance. The stability of the gas-like state
can be understood from a simple estimate of the energy per particle. For a contact
potential the interaction energy is given by (\ref{meanEcontact}) $E_{int}/N=g_{1D}
n g_2(0)/2$, where the
$g_2(0)=\langle\hat\Psi^\dagger(z)\hat\Psi^\dagger(z)\hat\Psi(z)\hat\Psi(z)\rangle/n^2$,
is the value at zero of the two-body correlation function (\ref{g2}) and
$\hat\Psi^\dagger$, $\hat\Psi$ are the creation and annihilation particle operators
(\ref{Psi}). In the limit $g_{1D}\to-\infty$ one can use for the correlation
function the result in the TG regime (\ref{g2TG})\cite{Gangardt03}, which does not
depend on the sign of $g_{1D}$. In the same limit the kinetic energy can be
estimated by (\ref{ETG}): $E_{kin}/N\simeq\pi^2\hbar^2n^2/(6m)$, corresponding to
the energy per particle of a TG gas. For the total energy $E=E_{kin}+E_{int}$ one
finds the result (\ref{Eexclud})
$E/N\simeq\pi^2\hbar^2n^2/(6m)-\pi^2\hbar^2n^3a_{1D}/(3m)$\label{HRdiscussion},
holding for $na_{1D}\ll 1$. For $na_{1D}<0.25$ this equation of state yields a
positive compressibility $mc^2=n\partial\mu/\partial n$, where $\mu=dE/dN$ is the
chemical potential and $c$ is the speed of sound, corresponding to a stable gas-like
phase. We will show that a more precise estimate gives that the gas-like state is
stable against cluster formation for $na_{1D}\lesssim 0.35$.

The analysis of the gas-like equation of state is carried out using the VMC
technique. The trial wavefunction employed in the calculation is of the form
(\ref{wfST}). For $g_{1D}<0$ ($a_{1D}>0$) the wavefunction $f(z)$ changes sign at a
nodal point which, for $\Rm\gg a_{1D}$, is located at $|z|=a_{1D}$. In the
attractive case the wavefunction has a node which means that the variational
calculation can be easily done, while without additional modifications the DMC can
not be done. The variational energy is calculated through the expectation value of
the Hamiltonian (\ref{Hamiltonian}) on the trial wave function (\ref{Eloc}). In the
calculations we have used $N=100$ particles with periodic boundary conditions and
because of the negligible dependence of the variational energy on the parameter
$\Rm$ we have used in all simulations the value $\Rm=L/2$, where $L$ is the size of
the simulation box. Calculations carried out with larger values of $N$ have shown
negligible finite size effects.

\section{Energy}

\begin{figure}[ht!]
\begin{center}
\includegraphics*[width=0.6\textwidth]{hr1.eps}
\caption{Energy per particle and compressibility as a function of the gas parameter $na_{1D}$. Solid symbols and
thick solid line: VMC results and polynomial best fit; thick dashed line: HR equation of state [Eq. (\ref{EHR})].
Thin solid and dashed line: compressibility from the best fit to the variational equation of state and from the HR
equation of state respectively.}
\label{figHR1}
\end{center}
\end{figure}

The results for the variational energy as a function of the gas parameter $na_{1D}$
are shown in Fig.~\ref{figHR1} with solid symbols. For small values of the gas
parameter our variational results agree very well with the equation of state of a
gas of hard-rods (HR) of size $a_{1D}$ (thick dashed line). The HR energy per
particle can be calculated exactly from the energy of a TG gas by accounting for the
excluded volume \cite{Girardeau60} (\ref{EHR}).

For larger values of $na_{1D}$, the variational energy increases with the gas
parameter more slowly than in the HR case and deviations are clearly visible. By
fitting a polynomial function to our variational results we obtain the best fit
shown in Fig.~\ref{figHR1} as a thick solid line. The compressibility obtained from
the best fit is shown in Fig.~\ref{figHR1} as a thin solid line and compared with
$mc^2$ of a HR gas (thin dashed line). As a function of the gas parameter the
compressibility shows a maximum and then drops abruptly to zero. The vanishing of
the compressibility implies that the system is mechanically unstable against cluster
formation. Our variational estimate yields $na_{1D}\simeq 0.35$ for the critical
value of the density where the instability appears. This value coincides with the
critical density for collapse calculated in the center of the trap for harmonically
confined systems \cite{Astrakharchik04,Astrakharchik04c}. It is worth noticing that
the VMC estimate of the energy of the system can be extended beyond the instability
point, as shown in Fig.~\ref{figHR1}. This is possible since the finite size of the
simulation box hinders the long-range density fluctuations that would break the
homogeneity of the gas. This feature is analogous to the one observed in the quantum
Monte-Carlo characterization of the spinodal point in liquid $^4$He
\cite{Boronat94}.

As shown in Fig.~\ref{figHR1}, the HR model describes accurately the equation of
state for small values of the gas parameter. A similar accuracy is therefore
expected for the correlation functions of the system. The correlation functions of a
HR gas of size $a_{1D}$ can be calculated from the exact wave function
\cite{Nagamiya40} (\ref{wf1DHR}). We calculate the static structure factor $S(k)$
(\ref{Sk}) and the one-body density matrix $g_1(z)$ (\ref{OBDM})

\section{One-body density matrix and static structure factor}

\begin{figure}[ht!]
\begin{center}
\includegraphics*[width=0.6\textwidth]{hr2.eps}
\caption{Static structure factor $S(k)$ for a gas of HR at different values of the gas parameter $na_{1D}$
(symbols) and for a TG gas (dashed line).}
\label{figHR2}
\end{center}
\end{figure}

Contrarily to the TG case, it is not possible to obtain analytical expressions for
$g_1(z)$ and $S(k)$ in the HR problem. We have calculated them using configurations
generated by a Monte Carlo simulation according to the exact probability
distribution function $|\psi_{HR}|^2$. The results for the static structure factor
are shown in Fig.~\ref{figHR2}. Compared to $S(k)$ in the TG regime, a clear peak is
visible for values of $k$ of the order of twice the Fermi wave vector $k_F=\pi n$
and the peak is more pronounced as $na_{1D}$ increases. The change of slope for
small values of $k$ reflects the increase of the speed of sound $c$ with $na_{1D}$.
The long-range behavior of $g_1(z)$ can be obtained from the hydrodynamic theory of
low-energy excitations \cite{Reatto67,Schwartz77,Haldane81}. For $|z|\gg\xi$, where
$\xi=\hbar/(\sqrt{2}mc)$ is the healing length of the system, one finds the
following power-law decay
%
\begin{equation}
g_1(z)\propto1/|z|^\alpha,
\label{OBDM1}
\end{equation}
%
where the exponent $\alpha$ is given by $\alpha=mc/(2\pi\hbar n)$. For a TG gas
$mc=\pi\hbar n$, and thus $\alpha_{TG}=1/2$. For a HR gas one finds
$\alpha=\alpha_{TG}/(1-na_{1D})^2$ and thus $\alpha>\alpha_{TG}$. This behavior at
long range is clearly shown in Fig.~\ref{figHR3} where we compare $g_1(z)$ of a gas
of HR with $na_{1D}=0.1$, 0.2 and 0.3 to the result of a TG gas \cite{Jimbo80}. The
long-range power-law decay of $g_1(z)$ is reflected in the infrared divergence of
the momentum distribution $n(k)\propto 1/|k|^{1-\alpha}$ holding for $|k|\ll 1/\xi$.
A gas of HR exhibits a weaker infrared divergence compared to a TG gas. The
correlation functions of a HR gas at $na_{1D}=0.1$, 0.2 should accurately describe
the physical situation of a Bose gas with large and negative $g_{1D}$. For
$na_{1D}=0.3$ we expect already some deviations from the HR model, as it is evident
from the equation of state in Fig.~\ref{figHR1}, which should broaden the peak in
$S(k)$ and decrease the slope of the power-law decay in $g_1(z)$ at large distances.
The analysis of correlation functions clearly shows that the super-Tonks regime
corresponds to a Luttinger liquid where short range correlations are significantly
stronger than in the TG gas.

\begin{figure}[ht!]
\begin{center}
\includegraphics*[width=0.6\textwidth]{hr3.eps}
\caption{One-body density matrix $g_1(z)$ for a gas of HR at different values of the gas parameter $na_{1D}$
(symbols) and for a TG gas (dashed line).}
\label{figHR3}
\end{center}
\end{figure}

\section{Collective modes}

Another possible experimental signature of the super-Tonks regime can be provided by
the study of collective modes. To this aim, we calculate the frequency of the lowest
compressional mode of a system of $N$ particles in a harmonic potential
$V_{ext}=\sum_{i=1}^N m\omega_z^2z_i^2/2$. We make use of LDA which allows us to
calculate the chemical potential of the inhomogeneous system $\tilde{\mu}$ and the
density profile $n(z)$ from the local equilibrium equation
$\tilde{\mu}=\mu[n(z)]+m\omega_z^2z^2/2$, and the normalization condition
$N=\int_{-R}^R n(z) dz$, where $R=\sqrt{2\tilde{\mu}/(m\omega_z^2)}$ is the size of
cloud. For densities $n$ smaller than the critical density for cluster formation,
$\mu[n]$ is the equation of state of the homogeneous system derived from the fit to
the VMC energies (Fig.~\ref{figHR1}). From the knowledge of the density profile
$n(z)$ one can obtain the mean square radius of the cloud $\langle
z^2\rangle=\int_{R}^R n(z)z^2 dz /N$ and thus, making use of the result
%
\cite{Menotti02}
\begin{equation}
\omega^2=-2\frac{\langle z^2\rangle}{d\langle z^2\rangle/d\omega_z^2} \;,
\label{cmode}
\end{equation}
%
one can calculate the frequency $\omega$ of the lowest breathing mode. Within LDA,
the result will depend only on the dimensionless parameter $Na_{1D}^2/a_z^2$, where
$a_z=\sqrt{\hbar/m\omega_z}$ is the harmonic oscillator length. For $g_{1D}>0$, {\it
i.e.} in the case of the LL Hamiltonian, the frequency of the lowest compressional
mode increases from $\omega=\sqrt{3}\omega_z$ in the weak-coupling mean-field regime
($Na_{1D}^2/a_z^2\gg 1$) to $\omega=2\omega_z$ in the strong-coupling TG regime
($Na_{1D}^2/a_z^2\ll 1$). The results for $\omega$ in the super-Tonks regime are
shown in Fig.~\ref{figHR4} as a function of the coupling strength. In the regime
$Na_{1D}^2/a_z^2\ll 1$, where the HR model is appropriate, we can calculate
analytically the first correction to the frequency of a TG gas. One finds the result
$\omega=2\omega_z [1+(16\sqrt{2}/15\pi^2)(N a_{1D}^2/a_z^2)^{1/2}+...]$.
Fig.~\ref{figHR4} shows that this expansion accurately describes the frequency of
the breathing mode when $Na_{1D}^2/a_z^2\ll 1$, for larger values of the coupling
strength the frequency reaches a maximum and drops to zero at $Na_{1D}^2/a_z^2\simeq
0.6$. The observation of a breathing mode with a frequency larger than $2\omega_z$
would be a clear signature of the super-Tonks regime.

\begin{figure}[ht!]
\begin{center}
\includegraphics*[width=0.6\textwidth]{hr4.eps}
\caption{Square of the lowest breathing mode frequency, $\omega^2$,
as a function of the coupling strength $Na_{1D}^2/a_z^2$ for the LL Hamiltonian
($g_{1D}>0$) and in the super-Tonks regime ($g_{1D}<0$). The dashed line is obtained
from the HR expansion (see text).}
\label{figHR4}
\end{center}
\end{figure}

\section{Conclusions}

In conclusion we have pointed out the existence of a strongly correlated regime in
quasi-1D Bose gases beyond the Tonks-Giradeau regime. This regime can be entered by
exploiting a confinement induced resonance of the effective 1D scattering amplitude.
We calculate the equation of state of the gas in the super-Tonks regime using VMC
and we estimate the critical density for the onset of instability against cluster
formation. The static structure factor and one-body density matrix are calculated
exactly within the hard-rod model, which provides the correct description of the
system for small values of the gas parameter. For harmonically trapped systems we
provide explicit predictions for the frequency of the lowest compressional mode.


==> BCSBEC.tex <==
\section{Calculation of the chemical potential from equation of state}

The chemical potential $\mu $ can be calculated by differentiating the
equation of state $\mu =\frac{\partial E}{\partial N}$. It is convenient to
measure the energy in units of fermi energy of an ideal gas per particle $%
E(N)=N~E_{F}{\cal E}(x)$, where $x=-(3\pi ^{2}Na^{3}/V)^{-1/3}~(N\frac{%
\partial E_{F}}{\partial N}=\frac{2}{3}E_{F},\frac{\partial x}{\partial N}=-%
\frac{1}{3}x)$%
\[
\tilde{\mu}=\frac{\mu }{\frac{5}{3}E_{F}}={\cal E}(x)-\frac{x}{5}{\cal E}%
^{\prime }(x)
\]

In the BEC limit one has%
\[
\tilde{\mu}=\frac{1}{5\,\pi \,}|x|^{-1}+\frac{32~\,0.6^{3}}{15\,\sqrt{6}{\pi
}^{\frac{3}{2}}\,}|x|^{-\frac{5}{2}}
\]

in the BCS limit instead one obtains

\[
\tilde{\mu}=1-\frac{4}{3\,\pi \,}x^{-1}+\frac{4(11-2\,\ln 2)}{15\,{\pi }^{2}}%
\,x^{-2}
\]

\section{Calculation of the compressibility from equation of state}

The sound velocity $c$ is related to the compressibility of the system%
\[
mc^{2}=n\frac{\partial \mu }{\partial n}
\]%
by denoting the energy per particle as $e(n)\ =E(n)/N$ and using the
definition of the chemical potential $\mu =\frac{\partial E}{\partial N}$we
obtain%
\[
mc^{2}=n\frac{\partial ^{2}}{\partial n^{2}}[n~e(n)]
\]

The natural parameter in the problem of BCS-BEC crossover is $%
x=-(k_{F}a)^{-1}=-(3\pi ^{2}na^{3})^{-1/3}$, the derivatives are $\frac{%
\partial x}{\partial n}=-\frac{1}{3}\frac{x}{n},$ $\frac{\partial ^{2}x}{%
\partial n^{2}}=\frac{4}{9}\frac{x}{n^{2}}$%
\begin{eqnarray*}
mc^{2} &=&2n\frac{\partial e(n)}{\partial n}+n^{2}\frac{\partial ^{2}e(n)}{%
\partial n^{2}}=2n\frac{\partial e}{\partial x}\frac{\partial x}{\partial n}%
+n^{2}\left[ \frac{\partial ^{2}e}{\partial x^{2}}\left( \frac{\partial x}{%
\partial n}\right) ^{2}+\frac{\partial e}{\partial x}\frac{\partial ^{2}x}{%
\partial n^{2}}\right] = \\
&=&-\frac{2}{3}xe^{\prime }+n^{2}\left[ e^{\prime \prime }\frac{1}{9}\frac{%
x^{2}}{n^{2}}+e^{\prime }\frac{4}{9}\frac{x}{n^{2}}\right] =-\frac{2}{9}%
xe^{\prime }+\frac{e^{\prime \prime }}{9}x^{2}
\end{eqnarray*}%
If we denote dimensionless energy ${\cal E}(x)=e(x)/E_{f},e(x)=\frac{3{\cal E%
}(x)}{10x^{2}}$%
\[
\tilde{c}^{2}=\frac{mc^{2}}{\frac{10}{9}E_{f}}={\cal E}(x)-\frac{3x}{5}{\cal %
E}^{\prime }(x)+\frac{x^{2}}{10}{\cal E}^{\prime \prime }(x)
\]

1) $x\ll 1,$ the BEC limit ${\cal E}(x)\ =-\frac{1}{6\pi x},{\cal E}^{\prime
}(x)=\frac{1}{6\pi x^{2}},{\cal E}^{\prime \prime }(x)=\allowbreak -\frac{1}{%
3\pi x^{3}},mc^{2}=-\frac{1}{3\pi x}$

2) $x\gg 1,$ the BCS\ limit ${\cal E}(x)=1-\frac{10}{9\pi x},{\cal E}%
^{\prime }(x)=\frac{10}{9\pi x^{2}},{\cal E}^{\prime \prime }(x)=-\frac{20}{%
9\pi x^{3}},mc^{2}=\frac{10}{9}-\frac{20}{9\,\pi \,x}$

In the BEC regime one can use equation of state for a bose gas of moleculas

\[
\frac{E/N}{E_{F}}=\frac{5}{18\pi |x|}\left( 1+\frac{128~0.6^{3/2}}{15%
\sqrt{6\pi ^{3}}}|x|^{-3/2}\right)
\]

this leads to the beyond mean-field corrections to the compressibility

\[
\frac{mc^{2}}{E_{F}}=\frac{0.6}{2\pi |x|}+\frac{8\,\,}{\sqrt{6\pi ^{5}}}%
\frac{0.6^{5/2}}{|x|^{5/2}}
\]

In the BCS\ limit the equation of state is%
\[
\frac{E/N}{E_{F}}=1-\frac{10}{9\pi x}+\frac{4}{21\pi ^{2}x^{2}}(11-2\ln 2)
\]

The next correction in the BCS\ regime is

\[
\frac{mc^{2}}{E_{F}}=\frac{10}{9}-\frac{20}{9\,\pi \,x}+\frac{176-32\,\ln 2}{%
27\,{\pi }^{2}\,x^{2}}
\]

\section{Fitting}

In order to calculate chemical potential and compressibility we fit our data
for the equation of state with a smooth function. Here we will describe the
construction of the fitting function.

Inspired by the construction procedure for the cubic splines we approximate
the equation of state by sum of power functions in different regions and
match them by imposing continuity of the function and its several
derivatives. Some of the coefficients of the power functions are readily
known from the analytic expansion in the BCS and BEC regimes.

The fitting function is following:%
\[
f(r)=\left\{
\begin{array}{cc}
\frac{a_{1}}{x}+\frac{a_{2}}{x^{2}}+\frac{a_{3}}{x^{3}}+\frac{a_{4}}{x^{4}},
& x<x_{1} \\
b_{0}+b_{1}x+b_{3}x^{3}+b_{5}x^{5}, & x_{1}<x\,<x_{2} \\
c_{0}+\frac{c_{1}}{x}+\frac{c_{2}}{x^{2}}+\frac{c_{3}}{x^{3}}+\frac{c_{4}}{%
x^{4}} & x_{2}<x%
\end{array}%
\right.
\]

where we have 15 parameters. Four parameters are known exactly%
\begin{eqnarray*}
a_{1} &=&-\frac{1}{6\pi } \\
c_{0} &=&1 \\
c_{1} &=&-\frac{10}{9\pi } \\
c_{2} &=&...
\end{eqnarray*}

Continuity conditions at the matching points for the funcion, its
derivative, second derivative and third derivative give 8 equations. Three
parameters are left free (for example $b_{0},~x_{1},~x_{2}$)and we fix them
by the least square fitting procedure.


==> Bethe.tex <==
In this Section the integral equations of exactly solvable bosonic and fermionic
one-dimensional models are presented. The equations were derived by using Bethe {\it
ansatz} method (see, for example, book \cite{Gaudin83}).
%\cite{Lieb63,Gaudin67,Yang67,Krivnov75,Casas91,Dunjko01}
%\cite{Gaudin67,Yang67,Casas91,}

\section{Lieb-Liniger equations}

A gas of repulsive bosons interacting via $\delta$-potential in one-dimensional
system is described by the Hamiltonian (\ref{LL}) with the relation between the
coupling constant $g_{1D}$ and the scattering length $a_{1D}$ given by (\ref{g1D}).
It was shown by Lieb and Liniger \cite{Lieb63} that the ground state energy can be
found from the solution of the integral equation (see for example,
\cite{Lieb63,Dunjko01}):
%
\begin{eqnarray}
\rho(k) =
\frac{1}{2\pi}
+\int\limits_{-1}^1\frac{2\lambda\rho(\varkappa)}{\lambda^2+(k-\varkappa)^2}\,\frac{d\varkappa}{2\pi}
\label{LLintegraleqs}
\end{eqnarray}

Normalization of the function $\rho(k)$ is related to the density $n|a_{1D}|$:
%
\begin{eqnarray}
%n|a_{1D}| = \int\limits_{-K}^K \rho(k)\,dk
\gamma = \frac{2}{n|a_{1D}|} = \int\limits_{-1}^1 \rho(k)\,dk,
\label{LLna1D}
\end{eqnarray}
%
here we use parameter $\gamma$ which is often introduced for solving the Bethe
equations and is inversely proportional to the density.

The energy per particle $E/N = n^2 e(n|a_{1D}|) \hbar^2/2m$ is obtained from integral
%
\begin{eqnarray}
%e(\gamma) = \frac{1}{n|a_{1D}|}\int\limits_{-K}^K k^2\rho(k)\,dk
e(n|a_{1D}|) = %\left(\frac{2}{\lambda\, n|a_{1D}|}\right)^3
\frac{\gamma^3}{\lambda^3}\int\limits_{-1}^1 k^2\rho(k)\,dk
\label{LLe}
\end{eqnarray}

The procedure of solving the integral equations can be following:
%
\begin{enumerate}
\item Fix some value of $\lambda$
\item Obtain $\rho(k)$ from (\ref{LLintegraleqs})
\item Obtain density $n|a_{1D}|$ from (\ref{LLna1D})
\item Obtain energy $e(n|a_{1D}|)$ from (\ref{LLe})
\end{enumerate}

\section{Attractive Fermi gas}

The Hamiltonain of a two-component fermi gas reads as follows:
%
\begin{eqnarray}
\hat H  =\left[
-\sum\limits_{i, \sigma}\frac{1}{2}\frac{\partial^2}{\partial z^2_{i,\sigma}}
+\frac{g_{1D}m}{\hbar^2n}\sum\limits_{i<j}^N\delta(z_{i,\uparrow}-z_{j,\downarrow})
\right]
\frac{\hbar^2n^2}{m}
\end{eqnarray}

In following we will express all energies in units of $\hbar^2 n^2/2m$ and all
distances in units of $|a_{1D}|$. Let us introduce notation $\gamma =
\frac{g_{1D}m}{\hbar^2n} >0$. The integral equation for the equation of state is
(see \cite{Krivnov75} with notation $\gamma=u/2$, $\rho=\sigma/2$):
%
\begin{eqnarray}
\rho(k)
= \frac{2}{\pi}
-\int\limits_{-K}^K\frac{2\gamma\,\rho(\varkappa)}{\gamma^2+(k-\varkappa)^2}
\,\frac{d\varkappa}{2\pi}
\end{eqnarray}

The density is
%
\begin{eqnarray}
na_{1D} = \int\limits_{-K}^K \rho(k)\,dk
\end{eqnarray}

The energy is
%
\begin{eqnarray}
e(\gamma) = \frac{1}{na_{1D}}\int\limits_{-K}^K k^2\rho(k)\,dk
-\frac{\gamma^2}{4}
\end{eqnarray}

\section{Repulsive Fermi gas}

This Hamiltonain can be solved for an arbitrary number of particles spin up
$N_{\uparrow}$ and spins down $N_\downarrow$. The corresponding integral equations
are ($\gamma = -\frac{2g_{1D}m}{\hbar^2n} >0$) \cite{Yang67}:
%
\begin{eqnarray}
\left\{
{\begin{array}{ccc}
\sigma(k) &=&
-\int\limits_{-B}^B\frac{2\gamma\sigma(\varkappa)}{\gamma^2+(k-\varkappa)^2}
\frac{d\varkappa}{2\pi}
+\int\limits_{-Q}^Q\frac{4\gamma\rho(y)}{\gamma^2+4(k-\varkappa)^2}
\frac{d\varkappa}{2\pi}\\
\rho(k) &=& 1+\int\limits_{-B}^B\frac{4\gamma\sigma(\varkappa)}{\gamma^2+4(k-\varkappa)^2}
\frac{d\varkappa}{2\pi}
\end{array}}
\right.
\label{Yang}
\end{eqnarray}

The limit $B\to\infty$ correspond to $N_\downarrow = N_\uparrow$. In this limit one
can simplify further the system of integral equations by introducing a Fourier
transformation (see also discrete lattice model \cite{Coll74}):
%
\begin{eqnarray}
\sigma(x) = \int\limits_{-\infty}^\infty e^{-ikx}\sigma(k)\frac{dk}{2\pi}\\
\sigma(k) = \int\limits_{-\infty}^\infty e^{ikx}\sigma(x)\,dx
\label{Fourier2}
\end{eqnarray}

By multiplying first equation from (\ref{Yang}) by $e^{-ikx}/2\pi$
and integrating over $k$ one obtains expression for the
$\sigma(x)$\footnote{
It is convenient to use following equality
$\int\limits_{-\infty}^\infty\frac{e^{\pm ikx}}{c^2+a^2(\varkappa-k)^2}
\frac{dk}{2\pi}=\frac{1}{2ac}e^{\pm i\varkappa x -\frac{c}{a}|x|}$
}

\begin{eqnarray}
\sigma(x) = \frac{1}{2\ch \frac{\gamma|x|}{2}} \int\limits_{-Q}^Q e^{-ikx}\rho(k)\frac{dk}{2\pi}
\label{sigma_k}
\end{eqnarray}

Setting $x=0$ one immediately sees that number of spin-down
particles is half of the total number of particles
$\int\sigma(k)\,dk = \frac{1}{2}\int\rho(k)\,dk$.

Inserting (\ref{Fourier2}) into second equation from (\ref{Yang}),
taking into account formula (\ref{sigma_k}) and carrying out two
integrations one obtains the integral equation involving only $\rho(x)$

\begin{eqnarray}
\rho(k) = \frac{1}{2\pi} + \int\limits_{-Q}^QK(k-\varkappa)\rho(\varkappa)\,\frac{d\varkappa}{2\pi},
\label{Repulsive fermions}
\end{eqnarray}

where the kernel is

\begin{eqnarray}
K(\xi) = %\frac{4c}{c^2+4\xi^2}-\frac{\pi}{c\ch \frac{\pi x}{c}}
2\int\limits_0^\infty \frac{\cos\xi x}{1+e^{\gamma x}}\,dx
\end{eqnarray}

Ones this equation is solved the density and energy are given by

\begin{eqnarray}
na_{1D} = \int\limits_{-Q}^Q\rho(k)\,dk,\\
e(\gamma) = \frac{1}{na_{1D}}\int\limits_{-Q}^Qk^2\rho(k)\,dk
\end{eqnarray}

Limits:

1) In the strongly interacting limit $\gamma\to\infty$ and the
kernel can be simplified

\begin{eqnarray}
K(\xi) = 2\int\limits_0^\infty \frac{\cos\xi x}{1+e^{\gamma x}}\,dx
=2\sum\limits_{n=1}^\infty (-1)^{n+1}
\int\limits_0^\infty \frac{\cos\xi x}{e^{n\gamma x}}\,dx
=2\sum\limits_{n=1}^\infty (-1)^{n+1}\frac{n\gamma}{(n\gamma)^2+\xi^2}
\approx\frac{2}{\gamma}\sum\limits_{n=1}^\infty \frac{(-1)^{n+1}}{n}
=\frac{2\ln 2}{\gamma}
\label{K1}
\end{eqnarray}

%$K(\xi)\approx
%2\int\limits_0^\infty \frac{\cos\xi x}{e^{cx}}\,dx=\frac{2c}{c^2+\xi^2}
%\approx\frac{2}{c} = 1$. One finds that
%$Q = \pi n(1-\frac{4n}{c})$, $\rho = \frac{1}{2\pi}(1+\frac{4n}{c})$.
The energy per particle in units of $\left[\frac{\hbar^2}{2ma^2}\right]$
is given by

\begin{eqnarray}
E = \frac{\pi^2 n^2}{3} - \frac{2\ln(2)\pi^3 n}{3}
\end{eqnarray}

which equals to the energy of gas of $N$ free fermions of the same
spin.

It is possible to express the kernel in terms of $\beta$-function
(see Gradstein-Ryzhik). Taking into account the series
representation $\beta(z) = \sum\limits_{k=0}^\infty\frac{(-1)^k}{z+k}$
one obtain following result from the (exact) sum (\ref{K1})

\begin{eqnarray}
K(\xi) = -\frac{1}{\gamma}\left(\beta\left(\frac{i\xi}{\gamma}\right)
+\beta\left(-\frac{i\xi}{\gamma}\right)\right).
\end{eqnarray}

The $\beta$-function is defined using the digamma function
$\beta(z) = \frac{1}{2}\left(\Psi(\frac{x+1}{2})
-\Psi(\frac{x}{2})\right)$ and digamma function is defined as
logarithmic derivative of the Gamma function
$\Psi(z) = \frac{\partial}{\partial z} \ln \Gamma(z)$.

The kernel can be expanded at small and large values of the
argument:

\begin{eqnarray}
K(\xi) = \frac{2}{\gamma}\ln 2 -\frac{3}{2\gamma^3} \xi^2 + {\cal O}(\xi^4),\\
K(\xi) = \frac{\gamma}{2}\xi^{-2} +\frac{2\gamma^3}{4}\xi^{-4} + {\cal O}(\xi^{-6})
\end{eqnarray}

%2) In the weakly interacting limit $c\to 0$ the second term of the
%kernel vanishes exponentially fast and can be neglected. In this
%limit the equation (\ref{Repulsive fermions}) can be rewritten in
%following way:
%
%\begin{eqnarray}
%2\pi \rho(x)-\int\limits_{-1}^1\frac{2 \frac{c}{2Q}}{\left(\frac{c}{2Q}\right)^2+(x-y)^2}\rho(y)\,dy = 1
%\end{eqnarray}
%
%This equation coincides with the Lieb-Liniger equation (\ref{LLintegraleqs})
%with the parameter $\lambda = c/2Q$.

\section{Numerical solution}

In the most general form the integral equations we have to solve is written as
%
\begin{eqnarray}
f(x)+\int\limits_{-Y}^Y K(x-y)f(y)\,dy = g(x),
\end{eqnarray}
%
where $f(x)$ is so far unknown solution, $K(x)$ is the kernel, $Y$ defines the
integration limit, $g(x)$ defines the normalization (in LL case it is constant). The
function $f(x)$ enters twice: once inside the integral and second time outside,
this can be remedied inserting the $\delta$-function:
%
\begin{eqnarray}
\int\limits_{-Y}^Y(\delta(x-y)+K(x-y))f(y)\,dy = g(x),
\label{BetheI}
\end{eqnarray}

Now we do discretization with spacing $\Delta x$. The equation (\ref{BetheI}) now
can be expressed in the matrix form:
%
\begin{eqnarray}
(I+K\Lambda) \vec f \Delta x = \vec g,
\end{eqnarray}
%
here $I$ stands for a unity matrix and the diagonal matrix $\Lambda$ is defined by
the integration method. Now the vector $f$ is obtained by multiplication of the
inverse matrix on $\vec g$:
%
\begin{eqnarray}
\vec f = \frac{1}{\Delta x} (I+K\Lambda)^{-1} \vec g,
\end{eqnarray}

For a uniform grid very good precision is achieved using the Simpson method. The
matrix $\Lambda$ in this case is defined as
$\Lambda = \mbox{diag}\{\frac13,\frac13,\frac43,\frac23,\frac43,...,
\frac43,\frac23,\frac43,\frac13\}$. The residual term of the integration is very
small and can be estimated as $I_{err} = \max f^{(4)}(x)\frac{(\Delta x)^5}{2880}$
and the error in the energy (which is defined by integrating the solution $f(x)$
with the weight proportional to $x^2$) is proportional to the spacing $\Delta x$ to
the forth power.

\newpage
\section{Expansions}

Energy expansion, unit of energy $\hbar^2/2ma_{1D}^2$:

\begin{eqnarray}
\nonumber
\begin{array}{|c|c|c|c|c|}
\hline
 term    & 0th & 1st & 2nd & 3rd\\
\hline
\hline
$Attractive gas: strong interaction$&\displaystyle
-1&\displaystyle
\frac{\pi^2(na_{1D})^2}{48}&\displaystyle
\frac{\pi^2(na_{1D})^3}{96}&\displaystyle
\frac{\pi^2(na_{1D})^4}{256}\\
\hline
$Attractive gas: weak interaction$&\displaystyle
\frac{\pi^2(na_{1D})^2}{12}&\displaystyle
-n|a_{1D}|&\displaystyle
-\frac{\ln^2(na_{1D}/2)}{\pi^2}&\\
\hline
$Repulsive gas: strong interaction$&\displaystyle
\frac{\pi^2(na_{1D})^2}{3}&\displaystyle
-\frac{2\ln(2) \pi^2(na_{1D})^3}{3}&&\\
\hline
$Repulsive gas: weak interaction$&\displaystyle
\frac{\pi^2(na_{1D})^2}{12}&\displaystyle
n|a_{1D}|&\displaystyle
&\\
\hline
\end{array}
\end{eqnarray}

Expansion of the chemical potential, unit of energy $\hbar^2/2ma_{1D}^2$:

\begin{eqnarray}
\nonumber
\begin{array}{|c|c|c|c|c|}
\hline
 term    & 0th & 1st & 2nd & 3rd\\
\hline
\hline
$Attractive gas: strong interaction$&\displaystyle
-1&\displaystyle
\frac{\pi^2(na_{1D})^2}{16}&\displaystyle
\frac{\pi^2(na_{1D})^3}{24}&\displaystyle
\frac{5\pi^2(na_{1D})^4}{256}\\
\hline
$Attractive gas: weak interaction$&\displaystyle
\frac{\pi^2(na_{1D})^2}{4}&\displaystyle
-2|na_{1D}|&\displaystyle
-\frac{\ln^2(na_{1D}/2)+2\ln(na_{1D}/2)}{\pi^2}\\
\hline
$Repulsive gas: strong interaction$&\displaystyle
\pi^2(na_{1D})^2&\displaystyle
-\frac{8\pi^2\ln(2) (na_{1D})^3}{3}&\\
\hline
$Repulsive gas: weak interaction$&\displaystyle
\frac{\pi^2(na_{1D})^2}{4}&\displaystyle
2|na_{1D}|&\displaystyle
&\\
\hline
$Lieb-Liniger gas: strong interaction$&\displaystyle
\pi^2(na_{1D})^2&\displaystyle
-\frac{8\pi^2}{3} (na_{1D})^3&\displaystyle
&\\
\hline
$gas of Hard-Rods (small density)$&\displaystyle
\pi^2(na_{1D})^2&\displaystyle
\frac{8\pi^2}{3} (na_{1D})^3&\displaystyle
&\\
\hline
\end{array}
\end{eqnarray}

The frequency of the oscillations
$\frac{\omega^2}{\omega_z^2} =4(1+\triangle\omega)$

\begin{eqnarray}
\nonumber
\begin{array}{|l|c|}
\hline
$limit$&\displaystyle
\triangle\omega\\
\hline
\hline
$Attractive gas: strong interaction$&\displaystyle
\frac{16\sqrt{2}}{15\pi^2} \frac{\sqrt{N}a_{1D}}{a_{z}}\\
\hline
$Attractive gas: weak interaction$&\displaystyle
\frac{8}{3\pi^2}/\frac{\sqrt{N}a_{1D}}{a_{z}}\\
\hline
$Repulsive gas: strong interaction$&\displaystyle
-\frac{32\sqrt{2}\ln 2}{15\pi^2} \frac{\sqrt{N}a_{1D}}{a_{z}}\\
\hline
$Repulsive gas: weak interaction$&\displaystyle
-\frac{8}{3\pi^2}/\frac{\sqrt{N}a_{1D}}{a_{z}}\\
\hline
$Lieb-Liniger gas: strong interaction$&\displaystyle
-\frac{32\sqrt{2}}{15\pi^2} \frac{\sqrt{N}a_{1D}}{a_{z}}\\
\hline
$Gas of Hard-Rods$&\displaystyle
\frac{32\sqrt{2}}{15\pi^2} \frac{\sqrt{N}a_{1D}}{a_{z}}\\
\hline
\end{array}
\end{eqnarray}

Speed of sound in units of $m/\pi\hbar n$

\begin{eqnarray}
\nonumber
\begin{array}{|c|c|c|c|c|}
\hline
 term    & 0th & 1st & 2nd & 3rd\\
\hline
\hline
$Attractive gas: strong interaction$&\displaystyle
\frac{1}{4} &\displaystyle
\frac{na_{1D}}{8}&\displaystyle
\frac{3(na_{1D})^2}{64} &\displaystyle
-\frac{3(na_{1D})^3}{128}\\
\hline
$Attractive gas: weak interaction$&\displaystyle
\frac{1}{2} &\displaystyle
-\frac{1}{\pi^2na_{1D}}&\displaystyle
\frac{\ln (2/na_{1D})-2}{\pi^4(na_{1D})^2}&\displaystyle
\\
\hline
$Repulsive gas: strong interaction$&\displaystyle
1&\displaystyle
-2\ln 2\, na_{1D}&&
\\
\hline
$Repulsive gas: weak interaction$&\displaystyle
\frac{1}{2}&\displaystyle
\frac{1}{\pi^2na_{1D}}&\displaystyle
&\\
\hline
\end{array}
\end{eqnarray}

Energy and chemical potential (LDA) in units of $N\hbar\omega_z$

\begin{eqnarray}
\nonumber
\begin{array}{|l|c|c|}
\hline
$limit$&\displaystyle \mu&\displaystyle E/N\\
\hline
\hline
$Repulsive gas: strong interaction$&\displaystyle
1-\frac{32\sqrt 2\ln 2}{9\pi^2}\frac{\sqrt{N}a_{1D}}{a_z}&\displaystyle
\frac{1}{2}\left(1-\frac{128\sqrt 2\ln 2}{45\pi^2}\frac{\sqrt{N}a_{1D}}{a_z}\right)\\
\hline
$Attractive gas: strong interaction$&\displaystyle
\frac{1}{4}\left(1+\frac{16\sqrt{2}}{9\pi^2}\frac{\sqrt N a_{1D}}{a_z}\right)&\displaystyle
\frac{1}{8}\left(1+\frac{64\sqrt{2}}{45\pi^2}\frac{\sqrt N a_{1D}}{a_z}\right)\\
\hline
$Repulsive: weak interaction$&\displaystyle
\frac{1}{2}\left(1+\frac{8}{\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)&\displaystyle
\frac{1}{4}\left(1+\frac{32}{3\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)\\
\hline
$Attractive gas: weak interaction$&\displaystyle
\frac{1}{2}\left(1-\frac{8}{\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)&\displaystyle
\frac{1}{4}\left(1-\frac{32}{3\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)\\
\hline
\end{array}
\end{eqnarray}

Size of the condensate and mean $z^2$ in units of $a_z^2$

\begin{eqnarray}
\nonumber
\begin{array}{|l|c|c|}
\hline
$limit$&\displaystyle R^2& z^2\\
\hline
\hline
$Repulsive gas: strong interaction$&\displaystyle
2N\left(1-\frac{32\sqrt 2\ln 2}{9\pi^2}\frac{\sqrt{N}a_{1D}}{a_z}\right)&\displaystyle
\frac{N}{2}\left(1-\frac{64\sqrt 2\ln 2}{15\pi^2}\frac{\sqrt{N}a_{1D}}{a_z}\right)\\
\hline
$Attractive gas: strong interaction$&\displaystyle
\frac{N}{2}\left(1+\frac{16\sqrt{2}}{9\pi^2}\frac{\sqrt N a_{1D}}{a_z}\right)&\displaystyle
\frac{N}{8}\left(1+\frac{32\sqrt{2}}{15\pi^2}\frac{\sqrt N a_{1D}}{a_z}\right)\\
\hline
$Repulsive: weak interaction$&\displaystyle
N\left(1+\frac{8}{\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)&\displaystyle
\frac{N}{4}\left(1+\frac{16}{3\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)\\
\hline
$Attractive gas: weak interaction$&\displaystyle
N\left(1-\frac{8}{\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)&\displaystyle
\frac{N}{4}\left(1-\frac{16}{3\pi^2}/\frac{\sqrt{N}a_{1D}}{a_z}\right)\\
\hline
\end{array}
\end{eqnarray}


==> GPperturb.tex <==

The main goal of the work is to calculate force acting on such an
object. Let us consider a small impurity which moves through the
condensate and can be described by by GPE. Consider a small
coupling constant of the impurity, then the equation can be
linearized. It is easy to obtain an equation for $\delta\psi$.

\begin{eqnarray}
i\hbar \frac{\partial }{\partial t}\delta \psi =\left( -\frac{\hbar ^{2}}{%
2m}\triangle -\mu +2g|\phi _{0}|^{2}\right) \delta \psi +g\phi
_{0}^{2}\,\delta \psi ^{\ast }+g_{i}\,\delta ({\bf r}-{\bf V}t)\phi _{0}
\end{eqnarray}

A similar equation is obtained for $\delta\psi^*$. The system of
the equations is solved by means of the Fourier transform.

\begin{equation}
\delta \psi _{{\bf k}}=g_{i}\phi _{0}\frac{\hbar {\bf k\cdot V}+\frac{%
\hbar ^{2}k^{2}}{2m}}{(\hbar {\bf k\cdot V})^{2}-\frac{\hbar
^{2}k^{2}}{2m}\left( \frac{\hbar ^{2}k^{2}}{2m}+2mc^{2}\right) }\ .
\end{equation}

In order to calculate the force you must write an equation for the
momentum conservation in the GPE (?). It is easy to obtain expression
for the force.

\begin{equation}
{\bf F}=-\int |\psi \left( {\bf r}\right) |^{2}\,\vec{\nabla}(g_{i}\delta
\left( {\bf r}\right) )\,d^{3}x=g_{i}(\vec{\nabla}|\psi({\bf r})|^{2})_{{\bf r}=0}
\end{equation}

You have to calculate the perturbation and at the point
of impurity the function is proportional to the coupling constant,
so the final answer is proportional to the coupling constant
squared.

By the way obtained equations contain more information, indeed we
can calculate the effective mass of this particle, which is related
to the suppression of the superfluidity by the presence of the
impurity and the result coincides with the one obtained from many
body Bogoliubov theory.

The point is that here it is important to use GPE. And if you would
like to solve this problem in hydrodynamics you will obtain
diverging expressions, which means that the important distances are
of the order of the correlation length.

The calculations in the GP framework can be produced and one obtain
the force. The answer is different for 3, 2, and 1- dimensional
systems. In $3D$ one can think of a laser beam moving an impurity,
in the $2D$ the laser beam itself can play a role of an impurity,
in $1D$ the thin (sharper than the healing length) knife-shaped
laser beam can cut the condensate.

\begin{eqnarray}
F_{V}^{3D}&=&4\pi nb^{2}mV^{2}(1-c^2/V^2)^2\\
F_{V}^{2D}&=&g_{i}^{2}n_{2}m^2(V^{2}-c^{2})/(2\hbar ^{3}V)\\
F_{V}^{1D}&=&2n_{1}\hbar ^{2}/mb_{1D}^{2}.
\end{eqnarray}

We have the Landau situation, the force is absent for velocities
smaller than the speed of sound. In $3D$ the force is quadratic in
velocity near the threshold. In the $2D$ the same behavior is
linear and in $1D$ it is a constant. But, of course, that can not
be applied for the regime of Tonks-Girardeau. We have to apply a
more delicate techniques.

The fact that in $1D$ system there is no dependence on the velocity
(of course, $V>c$) comes from particular properties of a
$\delta$-potential, namely that the Fourier transform of this
potential is a constant. Numerical solutions (Pavloff) for
finite-range potentials in $1D$ show no friction for $V<c$, maximal
friction for $V\ge c$ and smaller friction for $V\gg c$. Cases of
$\delta$-function, square-well and gaussian potentials were
considered. It was shown that the stationary solutions exist for\\
1) small values of $g_i$, or\\
2) very large or very small velocity\\
The movement with the velocity slightly smaller than the
speed of sound is always stationary for the repulsive interaction
and never for the attractive. In the latter case the drag force is
periodic in time and is almost sinusoidal for small density.

The dissipation energy can be calculated if we know the dynamic
form factor for $1D$ bose gas. If it is known the dissipation
energy is related to the Fourier transform of the interaction
potential.

\begin{equation}
Q=-\int\limits_{-\infty }^{\infty }\frac{dk}{2\pi }\int\limits_{0}^{\infty }%
\frac{d\omega }{\pi }\omega \frac{n_{1}}{2}S\left(\omega, k\right)
\left| U\left(\omega, k\right) \right| ^{2}
\end{equation}

For the $\delta$ interaction potential the contribution comes only
from frequencies $\omega = kV$.

\begin{equation}
\dot{E}=F_{V}V=-\frac{g_{i}^{2}n_{1}V}{\hbar }\int\limits_{0}^{\infty }
kS\left( kV,k\right)\frac{dk}{2\pi}
\end{equation}

Now we can immediately understand why the result for the
Tonks-Girardeau gas was wrong. Indeed, in order to have no
dissipation at small frequencies you must have $S$ which is zero at
small frequencies, but we know for the TG gas the dynamic form
factor vanishes not only at $k=0$, but also at $2k_F$ small
frequencies in the region $k\approx 2k_F$ will contribute to the
dissipation of the energy. In one-dimensional TG gas the friction
is different from zero and it is possible to show that the force is
proportional to the velocity of the impurity (?),
from this point of view the TG gas behaves as a normal liquid,
because if you move a body in a normal liquid the force is
proportional to the velocity.

Now we will consider the general case, which means not only
mean-field or TG gas, but also the region between. Actually we
will consider moderate MF, which means that the parameter $\gamma$
which defines nearness to the MF will be small enough, but not
zero.

Let us discuss what is the behavior of the dynamic form factor. It
tends to zero in a power-law way at small argument. But for us it
is not enough to know this behaviour, we also need to know it near
$2k_F$. We calculate it for any value of the parameter $\gamma$.
And it two limits: the MF and TG gas we can compare it to known
results.

We used generalization of the method introduced by Haldane in
1981. Let us discuss physics of the Haldane's picture. Consider a
$1D$ gas of N particles at zero temperature. If the quantum
fluctuations are switched off it will be a $1D$ crystal. The density
of $1D$ crystal is:

\begin{eqnarray}
\rho(x) = \sum\limits_{n}\delta\left(x-\frac{n}{\rho_0}\right)
\end{eqnarray}

where $\rho_0$ is the average density. It can be expressed in terms
of the Dirac's comb

\begin{eqnarray}
\rho(x) = \rho_0 + \rho_0 \sum\limits_{l=-\infty}^\infty
e^{i [l2\pi\rho_0 x]}
\end{eqnarray}

Now let us switch on the fluctuations. Of course, fluctuations at
small distances can not be described without using "very"
microscopic theory, but the fluctuations at large distances can be
described. The density in the presence of fluctuations is

\begin{eqnarray}
\rho(x) = \rho_0 + \rho_0 \sum\limits_{l=-\infty}^\infty
e^{i [l2\pi\rho_0 (x-u(x)]}
\end{eqnarray}

where $u$ is the displacement of an atom. It can be calculated if
position of each of the atoms in known.

\begin{eqnarray}
u = \frac{1}{\rho_0}\int\limits_0^x\delta\rho(x)\,dx
\end{eqnarray}

Of course, it is introduced for any distances, but what is
important is that we can use hydrodynamics to calculate it at large
distances.
%The density is canonically conjugate to the phase.
%It means that $x(\rho,t)$ $<>$
It is known that phonons can be averaged according to gaussian
distribution. So ..

\begin{eqnarray}
\langle\delta\rho(x,t)\delta\rho(0,0)\rangle
=A\rho_0^2 \langle e^{i(u(x,t)-u(0,0))}\rangle
=A \rho_0^2 e^{-\frac{1}{2}[\chi(0,0)-\chi(x,t)]}
\end{eqnarray}

%Coeff. -

Where $\chi(x,t)$ is the correlation function of $u(x,t)$

\begin{eqnarray}
\chi(x,t) = \langle u(x,t) u(0,0)\rangle
\end{eqnarray}

Once the correlation function is known, the dynamic structure
factor can be calculated by a Fourier transform.

The calculation of the correlation functions is based on the
Haldane's method, which, however, was developed for a stationary
case. We understood that the time dependence can be introduced
into this method. Also we recognized that we can obtain
more by this method, we can even calculate the exact coefficients
in the $S$.

Let us clarify the way the quantum fluctuations can be introduced.
The phonons exist in 1D. This description gives correct result
even for the extreme TG case. So we can express $\delta\rho$ in
terms of operator of creations and annihilations of phonons.

\begin{eqnarray}
\delta\rho = \sum_k \sqrt{\frac{\rho_0\hbar|k|}{2LMc}}
(\hat b_k e^{i(kx-\omega t)}+\hat b^\dagger_k e^{-(ikx-\omega t)})
\label{rho}
\end{eqnarray}

The problem is that the integration over $k$ converges at small
$k$, but diverges at large $k$. This logarithmic divergence can be
avoided by truncating at distances of the order of the correlation
length. The result is

\begin{eqnarray}
\frac{\langle\hat\rho(x,t)\hat\rho(0,0)\rangle}{\rho_0^2}
= 1+\frac{\hbar}{4\pi Mc\rho_0}
\left(\frac{1}{(x+ct)^2} + \frac{1}{(x-ct)^2}\right)
+
2\sum\limits_{m=1}^\infty
C_i\cos(2\pi m\rho_0 x)\left(\frac{x^2-c^2t^2}{\xi^2}\right)^{-\frac{\eta}{2}}
\label{corr}
\end{eqnarray}

The result lead to important conclusions. First of all one can see
the oscillations. Second, the behavior is governed by the parameter
$\eta$. Parameter $\eta$ is the most important parameter in the
theory of $1D$ bose gas.

\begin{eqnarray}
\eta = \frac{2p_F}{c}
\end{eqnarray}

The parameter goes to infinity when we move into MF regime.
Instead in TG regime it is finite and equals $2$.

Before going further following thing should be pointed out. The
calculation was produced with logarithmic accuracy which means that
the coefficient in the front will not be defined. And that can not
be improved in general, because the result depends not only on the
large distance behavior which can be described by hydrodynamics,
but also on small distances. But if the parameter $\eta$ is large
and we are close to the mean field regime, the situation is
different. The point is following, the hydrodynamic description is
valid for distances large compared to the healing length, but we do
have a description for distances of the order of the healing
length, and even more. According to paper of Popov it is possible
to use hydrodynamics in full range of Bogoliubov's theory.
%Bogoliubov's theory in some sense is a hydrodynamic theory.
The only difference is that in all equations we must change the
velocity of sound $c$ on Bogoliubov's velocity $\omega_{bog}/k$. If
you make this substitution, which is completely correct thing to do
you will find all integrals to be convergent. When if the parameter
$\eta$ equals $2$ you also know the answer. This is the
Tonks-Girardeau gas.

The result is following

\begin{eqnarray}
\frac{\langle\hat\rho(x)\hat\rho(0)\rangle}{\rho_0^2}
= 1+
2\sum\limits_{m=1}^\infty
\frac{\cos(2\pi m\rho_0 x)}{(4C)^{\eta m^2}}
\left(\frac{\hbar}{Mcx}\right)^{\eta m^2},
\label{our Sxt}
\end{eqnarray}

where $C = e^\gamma \approx 1.781$.

You can see that there are strong oscillations. Oscillations have
infinite amplitude from the values of momenta which are multiple of
$2k_F$. This means that in the Fourier space (which is the
structure factor) there will be zeros at $2k_F$.

The main difficulty was to perform the Fourier transform. We
are interested in the structure factor near $2k_F$

\begin{eqnarray}
S(k, \omega) = \sum\limits_{m=1}^\infty \frac{8\pi^2\rho_0 c}{\hbar\Gamma^2\left(\frac{m^2\eta}{2}\right)}
\left(\frac{\hbar}{8CMc^2}\right)^{m^2\eta}
\left[(\omega^2 - c^2(k-2mk_F)^2)^{\frac{m^2\eta}{2}-1}
+(\omega^2 - c^2(k+2mk_F)^2)^{\frac{m^2\eta}{2}-1}\right]
\end{eqnarray}








\chapter{Calculation of the superfluid fraction and the energy dissipation from the GPE}
\section{Calculation of the superfluid fraction in a homogeneous system \label{sec1}}

The Gross-Pitaevskii equation %(\ref{Gross-Pitaevskii})
for the condensate wave function in the absence of external field takes the form

\begin{eqnarray}
i\hbar\frac{\partial }{\partial t} \psi({\bf r}, t) =
\left(-\frac{\hbar^2}{2m} \triangle + g|\psi({\bf r}, t)|^2\right)
\psi({\bf r}, t)
\label{GP}
\label{GPE}
\end{eqnarray}

Let us add a moving impurity that creates an external field
$V_{ext}({\bf r}, t) = \gi \delta({\bf r - V}t)$ and let us
treat it as a perturbation to the solution $\phi_0({\bf r}, t)$ of
the equation (\ref{GP}), {\it i.e.}

\begin{eqnarray}
\psi({\bf r}, t) = \left[\phi_0({\bf r}) + \delta\psi({\bf r}, t)\right]
\exp\left(-i \frac{\mu t}{\hbar} \right),
\label{expansion}
\end{eqnarray}

Then, substitution of (\ref{expansion}) into (\ref{GP}) gives

\begin{eqnarray}
i\hbar\frac{\partial }{\partial t} \delta \psi =
\left(-\frac{\hbar^2}{2m} \triangle - \mu\right) \delta \psi
+ 2 g|\phi_0|^2 \delta \psi
+ g \phi_0^2 \delta \psi^*
+ \gi \delta ({\bf r - V}t) \phi_0
\label{first approx}
\end{eqnarray}

The perturbation follows the moving impurity, so
$\delta \psi$ is a function of ${\bf r - V}t$.

Let us introduce the new variable ${\bf r' = r - V}t$. %and fix the time.
It means that the coordinate derivative can be related to time derivative

\begin{eqnarray}
\frac{\partial}{\partial t} \delta \psi({\bf r - V}t)& =&
-{\bf V \nabla} \delta \psi({\bf r - V}t), \label{dt2nabla}\\
\triangle {\bf r'} &=& \triangle {\bf r}
\end{eqnarray}

and instead of (\ref{first approx}) one has

\begin{eqnarray}
\left( i\hbar {\bf V \nabla} - \frac{\hbar^2}{2m} \triangle
- \mu + 2 g|\phi_0|^2 \right) \delta \psi
+ g \phi_0({\bf r})^2 \delta \psi^*
+ \gi \delta ({\bf r}) \phi_0 = 0,
\end{eqnarray}

(from now on, the subscript over ${\bf r}$ will be dropped)

Taking the Fourier transform of this equation and treating $\phi_0$
as a real constant ({\it i.e.} the solution for the uniform case
$g\phi_0^2 = \mu = mc^2$) one obtains

\begin{eqnarray}
\left( -\hbar {\bf k V} + \frac{\hbar^2k^2}{2m}
+ mc^2 \right) \delta \psi_k
+ mc^2 (\delta \psi_{-k})^*
 + \gi \phi_0 = 0,
\label{Fourier}
\end{eqnarray}

where we used the property of Fourier components
$\delta (\psi^*)_{k} = \delta (\psi_{-k})^*$.

The substitution of $(-{\bf k})$ in the equation complex
conjugate of (\ref{Fourier}) gives

\begin{eqnarray}
mc^2\,\delta \psi_{k}
+ \left( \hbar {\bf k V} + \frac{\hbar^2k^2}{2m}
+ mc^2 \right) (\delta \psi_{-k})^*
+ \gi \phi_0 = 0
\label{Fourier conjugate}
\end{eqnarray}

The solution for the system of linear equations
(\ref{Fourier} - \ref{Fourier conjugate}) is given by

\begin{eqnarray}
\delta \psi_{k}
= -\frac{\gi \left(\hbar{\bf k V} + \frac{\hbar^2 k^2}{2m}\right)\phi_0}
{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2 k^2}{2m}+2\mu\right)
-(\hbar{\bf k V})^2}
\label{dPsi}
\end{eqnarray}


\newpage
\section{Energy dissipation}

The force $\overline{\bf F}$ that acts on the moving perturbation in the frame moving
with the perturbation is given by

\begin{eqnarray}
\overline{\bf F} =
\int\!\! {\bf F(r)}\,|\psi({\bf r})|^2\,{\bf dr} =
-\int\!\! \vec\nabla U({\bf r})\,|\psi({\bf r})|^2\,{\bf dr} =
-\left.U({\bf r}) |\psi({\bf r})|^2\right|_{boundary}+
\int\!\! U({\bf r}) \vec{\nabla} |\psi({\bf r})|^2\,{\bf dr}
\end{eqnarray}

We consider a short-correlated interaction potential
$U({\bf r}) = \gi \delta({\bf r})$. It is equal to zero on the
boundaries, so we have only one term

\begin{eqnarray}
\begin{array}{lcl}
\overline{\bf F} & = &
\int \gi \delta({\bf r}) \vec{\nabla} |\psi({\bf r})|^2 {\bf dr}
= \int \gi \delta({\bf r}) \vec{\nabla} |\phi_0({\bf r})+\delta\psi({\bf r})|^2{\bf dr}\approx\\
&\approx&
\int \gi \delta({\bf r})
\left(
\vec{\nabla}|\phi_0|^2
+(\vec{\nabla} \phi_0^*)\delta\psi+(\vec{\nabla} \phi_0)\delta\psi^*
+\psi^*_0 (\vec{\nabla} \delta\psi)+\phi_0 (\vec{\nabla} \delta\psi^*)
\right){\bf dr}
\end{array}
\end{eqnarray}

In a homogeneous system the unperturbed wave function is a
constant $\phi_0 = \sqrt{n}$, so $\vec{\nabla}\phi_0 = 0$ and only
following contribution remains

\begin{eqnarray}
\begin{array}{lcl}
\overline{\bf F} & = &
\int \gi \delta({\bf r})\phi_0 \vec{\nabla} (\delta\psi({\bf r})+\delta\psi^*({\bf r}))
\,{\bf dr}=\\
&=& \gi\phi_0(0) \int \delta({\bf r})\vec{\nabla}
\left(\int e^{i{\bf kr}}[\delta\psi_k + (\delta\psi^*)_k]\,\frac{\bf dk}{(2\pi)^3}
\right)\,{\bf dr}=
\gi\phi_0 \int i{\bf k}[\delta\psi_k + (\delta\psi_{-k})^*]\,\frac{\bf dk}{(2\pi)^3}
\end{array}
\label{x}
\end{eqnarray}

Here we used the property of Fourier components
$\delta (\psi^*)_k = \delta (\psi_{-k})^*$.
Let us insert the expression for $\delta \psi_k$ (\ref{dPsi})
into formula (\ref{x})

\begin{eqnarray}
\overline{\bf F} =
-\gi\phi_0 \int i{\bf k}
\frac{2\gi \frac{\hbar^2 k^2}{2m}\phi_0}
{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2 k^2}{2m}+2mc^2\right)
-(\hbar{\bf k V})^2}
\,\frac{\bf dk}{(2\pi)^3} =
\label{gppertF}
\end{eqnarray}

\begin{eqnarray} =
2(\gi\phi_0)^2 \int
\frac{ i{\bf k} \frac{\hbar^2 k^2}{2m}}{2\hbar{\bf k V}}
\left[
\frac{1}{\hbar{\bf k V}-\sqrt{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2 k^2}{2m}+2mc^2\right)}}
+\frac{1}{\hbar{\bf k V}+\sqrt{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2 k^2}{2m}+2mc^2\right)}}
\right]
\,\frac{\bf dk}{(2\pi)^3}
\end{eqnarray}

We will add small positive imaginary part to the momentum
${\bf kV} \to {\bf kV} + i\varepsilon$ in order to go around the pole from above and
will take use of the Sokhotskii formula

\newpage
\begin{figure}
\includegraphics[width=0.3\textwidth]{Contour.eps}
\caption{Integration contour}
\label{Contour}
\end{figure}

\begin{eqnarray}
\frac{1}{x+i\varepsilon} = {\cal P}\frac{1}{x} - i\pi\delta(x)
\end{eqnarray}

The part of the integral taken in the sense of the principal value
is real and could provide only nonphysical imaginary contribution to the force,
thus we conclude that only $\delta$-function contributes to the
integral

\begin{eqnarray}
2(\gi\phi_0)^2 \int
\frac{i{\bf k}\frac{\hbar^2 k^2}{2m}(-i\pi)}{2\hbar{\bf k V}}
\mbox{\small $
\left[
\delta\!\left(\hbar{\bf k V}\!\!-\!\!\sqrt{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2
k^2}{2m}\!+\!2mc^2\right)}\right)
\!+\!\delta\!\left(\hbar{\bf k V}\!\!+\!\!\sqrt{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2
k^2}{2m}\!+\!2mc^2\right)}\right)
\right]$}
\,\frac{\bf dk}{(2\pi)^3}
\label{y}
\end{eqnarray}

It is convenient to do the integration in spherical coordinates
with $\vartheta$ being angle between $\bf k$ and $\bf V$. There is
no dependence on the angle $\phi$ and it can be immediately
integrated out

\begin{eqnarray}
\int f({\bf k})\,{\bf dk} =
\int\limits_{-\infty}^{\infty}\!\!\int\limits_0^\pi
f(k, \vartheta)\,2\pi k^2 \sin \vartheta \; dk d\vartheta
= \int\limits_{-\infty}^{\infty}\int\limits_{-1}^1
f(k, \vartheta)\,2\pi k^2 dk d(\cos\vartheta)
\end{eqnarray}

The $\delta$-function can be further developed

\begin{eqnarray}
\delta\left(\hbar{\bf k V}\pm\sqrt{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2
k^2}{2m}+2mc^2\right)}\right) =
\frac{1}{\hbar kV}\delta\left(\cos\vartheta\pm
\frac{1}{\hbar kV}\sqrt{\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2
k^2}{2m}+2mc^2\right)}\right)
\end{eqnarray}

This formula defines maximal momentum $k_{max}$ which can contribute to the
integral. Condition $|\cos\varphi| \le 1$ gives

\begin{eqnarray}
\frac{\hbar^2 k_{max}^2}{2m} = 2m(V^2-c^2)
\label{kmax}
\end{eqnarray}

Now it is evident that the effect is present only in a motion with speed larger
then the speed of sound.

Let us calculate the projection $F_V$ of the force $\overline{\bf F}$ to
the direction $\bf V$of the movement of the perturbation. It means
that we have to multiply formula (\ref{y}) on ${\bf V}/V$

\begin{eqnarray}
F_V =
(\gi\phi_0)^2~2\!\!\!\!\!\!\!\!\int\limits_0^{2m(V^2-c^2)}
\frac{\frac{\hbar^2 k^2}{2m}\pi}{\hbar V}
\frac{1}{\hbar kV} \frac{2\pi k^2dk}{(2\pi)^3} =
\frac{(\gi\phi_0)^2}{4\pi \hbar^2 V^2}
\int\limits_0^{2m(V^2-c^2)}\frac{\hbar^2 k^2}{2m}2kdk =
\end{eqnarray}

\begin{eqnarray}
=\frac{(\gi\phi_0)^2}{4\pi \hbar^2 V^2}\frac{2m}{\hbar^2}
\int\limits_0^{2m(V^2-c^2)}\frac{\hbar^2 k^2}{2m}
d\left(\frac{\hbar^2 k^2}{2m}\right)
=\frac{(\gi\phi_0)^2m}{2\pi \hbar^4 V^2}
\frac{1}{2}\left(2m(V^2-c^2)\right)^2
\end{eqnarray}

Now we can use that square of the unperturbed wave function gives the density
$\phi_0^2 = n$ and the coupling constant can be expressed as

\begin{eqnarray}
\gi = \frac{4\pi\hbar^2 a}{m}
\end{eqnarray}

Finally, we obtain following expression for the projection of the force

\begin{eqnarray}
F_V = 16\pi na^2 mV^2 \left(1-\frac{c^2}{V^2}\right)^2
\label{F3D}
\end{eqnarray}

\begin{figure}
\includegraphics[width=0.6\textwidth]{Force.eps}
\caption{Force}
\end{figure}

\section{Energy dissipation in low dimensional systems}

The Fourier components of the perturbed wave function $\delta\psi_k$
are given by the formula (\ref{dPsi}), which is valid for all
number of dimensions.

The expression for the force acting on the system is given by (\ref{gppertF}), where
${\bf k}/(2\pi)^3$ must be replaced according to the number of dimensions $D$.

\begin{eqnarray}
F_V =
\frac{2i\gi^2\phi_0^2}{V}
\int \frac{{\bf k V} \frac{\hbar^2 k^2}{2m}}
{(\hbar{\bf k V})^2-\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2 k^2}{2m}+2mc^2\right)}
\,\frac{\bf dk}{(2\pi)^D}
\end{eqnarray}

\subsection{Two-dimensional system}

In two dimensions one has
${\bf dk} = k dk d\vartheta = - \frac{k}{\sqrt{1-\cos^2\vartheta}} dk\,d\!\cos\vartheta$
and projection of the force ${\bf F}$ on the direction of the movement
${\bf V}$ is equal to

\begin{equation}
\begin{array}{l}
\displaystyle
F^{2D}_V =
-\frac{2ig^2_{imp}\phi_0^2}{V}
\int\limits_0^\infty \int\limits_{-1}^1
 \frac{kV\cos\vartheta \frac{\hbar^2 k^2}{2m}}
{(\hbar kV \cos\vartheta )^2-\frac{\hbar^2 k^2}{2m} \left(\frac{\hbar^2 k^2}{2m}+2mc^2\right)}
\frac{k}{\sqrt{1-\cos^2\vartheta}}
\frac{dk\,d\!\cos\vartheta}{(2\pi)^2} =\\
\displaystyle=-\frac{i\gi^2 n}{8\pi^2 mV^2}
\int\limits_0^\infty \int\limits_{-1}^1
\left(\frac{1}{\cos\vartheta + \sqrt{\left(\frac{\hbar^2k^2}{2m}+2mc^2\right)/2mV^2}}
+\frac{1}{\cos\vartheta - \sqrt{\left(\frac{\hbar^2k^2}{2m}+2mc^2\right)/2mV^2}}\right)
\frac{k^2\,dk\,d\!\cos\vartheta}{\sqrt{1-\cos^2\vartheta}}
\end{array}
\end{equation}

The integral is different from zero only if integrand has poles,
which means that the velocity $V$ must be larger than the speed of
sound $c$. Only momenta smaller than $k_{max}$ (see eq.(\ref{kmax}))
contribute to the integral. Path of the integration is same as on
the figure (\ref{Contour}) and the integral equals

\begin{eqnarray}
F^{2D}_V
= -\frac{i\gi^2n}{8\pi^2mV^2}
\int\limits_0^{k_{max}}
\frac{2\pi i k^2\,dk}
{\sqrt{1-\left(\frac{\hbar^2k^2}{2m}+2mc^2\right)/2mV^2}}
= \frac{\gi^2n}{4\pi mV^2}
\int\limits_0^{k_{max}}
\frac{2mV k^2\,dk}
{\hbar\sqrt{\frac{4m^2(V^2-c^2)}{\hbar^2}-k^2}}
\end{eqnarray}

We recall simple integral equality
$\int_0^\varkappa\frac{k^2\,dk}{\sqrt{\varkappa^2-k^2}}
= \frac{\pi}{4}\varkappa^2$ and finally have

\begin{eqnarray}
F^{2D}_V = \frac{\gi^2 n}{2\hbar^3V}(V^2-c^2)
\end{eqnarray}

In a quasi two dimensional system, {\it i.e.} when motion in
one of the dimensions is frozen to the ground state of a
harmonic oscillator confinement, the coupling constant
equals $\gi = \sqrt{2\pi}\frac{\hbar^2a}{ma_{osc}}$
(see derivation (\ref{gimp2D}))
and the force can be expressed in terms of the three dimensional
scattering length and the oscillator length

\begin{eqnarray}
F^{2D}_V = \pi n\hbar V \frac{a^2}{a^2_{osc}} \left(1-\frac{c^2}{V^2}\right)
\label{F2D}
\end{eqnarray}

On the contrary to the three dimensional case (\ref{F3D}), in two
dimensions the force acting on the system does not depend
on the mass of the gas particles.


\section{Beyond mean-field corrections to the energy in low dimensional systems}

The "beyond mean-field" correction to the ground-state energy ($V = 0$)
is given by formula

\begin{eqnarray}
dE^{(2)} = \gi^2n\int\frac{2mc^2}{\frac{\hbar^2k^2}{2m}
\left(\frac{\hbar^2k^2}{2m}+2mc^2\right)}\frac{d^Dk}{(2\pi)^D}
\end{eqnarray}

It is convenient to rewrite in following form

\begin{eqnarray}
dE^{(2)} =
\frac{\gi^2n(2m)^3c^2}{\hbar^4}
\int\frac{1}{k^2\left(k^2+\left(\frac{2mc}{\hbar}\right)^2\right)}
\frac{d^Dk}{(2\pi)^D}
\end{eqnarray}

\subsection{two dimensional system}

In two dimensions the integral has logarithmic divergence at small
momenta

\begin{eqnarray}
dE^{(2)}_{2D} =
\frac{\gi^2n(2m)^3c^2}{\hbar^4}
\int\limits_0^\infty\frac{1}{k\left(k^2+\left(\frac{2mc}{\hbar}\right)^2\right)}
\frac{dk}{(2\pi)^2}
\end{eqnarray}

\subsection{one dimensional system}

The principal value of the integral (the Riemann integral does not
exist due to divergence at $k = 0$) is finite, but negative.

\begin{eqnarray}
dE^{(2)}_{1D} =
\frac{\gi^2n(2m)^3c^2}{\hbar^4}
\int\limits_{-\infty}^\infty\frac{1}{k^2\left(k^2+\left(\frac{2mc}{\hbar}\right)^2\right)}\frac{dk}{2\pi} =\\
=\frac{\gi^2nm}{\pi\hbar^2}\int\limits_{-\infty}^\infty\left(\frac{1}{k^2}-\frac{1}{k^2+\left(\frac{2mc}{\hbar}\right)^2}\right)\,dk
= -\frac{\gi^2n}{2\hbar c}
\end{eqnarray}


